Hamiltonian-based Neural ODE Networks on the SE(3) Manifold For Dynamics Learning and Control

Accurate models of robot dynamics are critical for safe and stable control and generalization to novel operational conditions. Hand-designed models, however, may be insufficiently accurate, even after careful parameter tuning. This motivates the use of machine learning techniques to approximate the robot dynamics over a training set of state-control trajectories. The dynamics of many robots, including ground, aerial, and underwater vehicles, are described in terms of their SE(3) pose and generalized velocity, and satisfy conservation of energy principles. This paper proposes a Hamiltonian formulation over the SE(3) manifold of the structure of a neural ordinary differential equation (ODE) network to approximate the dynamics of a rigid body. In contrast to a black-box ODE network, our formulation guarantees total energy conservation by construction. We develop energy shaping and damping injection control for the learned, potentially under-actuated SE(3) Hamiltonian dynamics to enable a unified approach for stabilization and trajectory tracking with various platforms, including pendulum, rigid-body, and quadrotor systems.

==> tex/NikolaysAddon.tex <==
\section{Nikolay's Addon}
\label{sec:nikolay}

% the generalized mass matrix $\bfM$ is constant with respect to the generalized system coordinates $(\mathbf\frakq$ and 

We extend the interconnection and damping assignment passivity-based control approach (IDA-PBC) to achieve under-actuated trajectory tracking over the SE(3) manifold for Port-Hamiltonian systems. Let $\bfx^*(t) = (\mathbf\frakq^*(t), \mathbf\frakp^*(t))$ be a desired state trajectory that the system should track. We develop an IDA-PBC controller utilizing both potential and kinetic energy shaping and feedforward terms based on the time-derivative of the desired moment $\mathbf\frakp^*(t)$. 






==> tex/unused.tex <==
\section{Unsued text from controller}










\subsection{Old text}



 Let $\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp)$ be the desired Hamiltonian:
\begin{equation}
\label{eq:desired_hamiltonian}
\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp) = \frac{1}{2}(\mathbf\frakp - \mathbf\frakp^*)^\top \bfM_d^{-1}(\mathbf\frakq)(\mathbf\frakp - \mathbf\frakp^*) + \bfV_d(\mathbf\frakq),
\end{equation}
where $\bfM_d(\mathbf\frakq)$ is the desired generalized mass and $\bfV_d(\mathbf\frakq)$ is the desired generalized potential energy such that $\bfx^* = \text{argmin}\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp)$. The state-feedback control input $\bfu$ is decomposed into energy-shaping and damping-injection components: $\bfu_{ES}(\mathbf\frakq, \mathbf\frakp)$, and $\bfu_{DI}(\mathbf\frakq, \mathbf\frakp)$, respectively. The control input  $\bfu$ is to shape the Port-Hamiltonian dynamics in Eq. \eqref{eq:port_Hal_dyn} into the desired form~\cite{van2014port,ortega2002stabilization}:
\begin{equation}
\label{eq:desired_port_Hal_dyn}
\begin{bmatrix}
\dot{\mathbf\frakq} \\
\dot{\mathbf\frakp} \\
\end{bmatrix}
= (\bf\mathcal{J}_d(\mathbf\frakq, \mathbf\frakp) - \bf\mathcal{R}_d(\mathbf\frakq, \mathbf\frakp))
\begin{bmatrix}
\frac{\partial \mathcal{H}_d}{\partial \mathbf\frakq} \\
\frac{\partial \mathcal{H}_d}{\partial \mathbf\frakp} 
\end{bmatrix},
\end{equation}
where 
\begin{equation}
\label{eq:desired_JR}
\begin{aligned}
\bf\mathcal{J}_d &=& \begin{bmatrix}
\bf0 & \mathbf\frakq^{\times}\bfM^{-1}(\mathbf\frakq)\bfM_d(\mathbf\frakq) \\
-\bfM_d(\mathbf\frakq)\bfM^{-1}(\mathbf\frakq)\mathbf\frakq^{\times\top} & \bfJ_{2}(\mathbf\frakq, \mathbf\frakp) \end{bmatrix},\\
\bf\mathcal{R}_d &=& \begin{bmatrix}
\bf0 & \bf0 \\
\bf0 &\bf\bfK_d
\end{bmatrix}.  
\end{aligned}
\end{equation}
The matrix $\bfJ_{2}(\mathbf\frakq, \mathbf\frakp)$ and the desired mass $\bfM_d(\mathbf\frakq)$ satisfy the matching equations:
\begin{eqnarray}
\bf\mathcal{G}^\perp\left(\mathbf\frakq^{\times\top}\frac{\partial \mathcal{H}}{\partial \mathbf\frakq} - \mathbf\frakp^{\times}\frac{\partial \mathcal{H}}{\partial \mathbf\frakp} + \bfJ_{2}(\mathbf\frakq, \mathbf\frakp)\frac{\partial \mathcal{H}_d}{\partial \mathbf\frakp} \right.&&\nonumber \\
-\left.\bfM_d(\mathbf\frakq)\bfM^{-1}(\mathbf\frakq)\mathbf\frakq^{\times\top}\frac{\partial \mathcal{H}_d}{\partial \mathbf\frakq}\right) &=& 0. \label{eq:idapbc_matching}
\end{eqnarray}
The matrix $\bfJ_{2}(\mathbf\frakq, \mathbf\frakp)$ is commonly considered free to choose and the desired generalized mass $\bfM_d(\mathbf\frakq)$ is found by solving the partial derivative equation (PDE) \eqref{eq:idapbc_matching}.

Given $\bfJ_{2}(\mathbf\frakq, \mathbf\frakp)$ and $\bfM_d(\mathbf\frakq)$, the energy-shaping and damping-injection control inputs are obtained as:
\begin{eqnarray}
\bfu_{ES}(\mathbf\frakq, \mathbf\frakp) &=& \bfg^{\dagger}(\mathbf\frakq)\left(\bfR^{\times\top}\frac{\partial \mathcal{H}}{\partial \mathbf\frakq} - \mathbf\frakp^{\times}\frac{\partial \mathcal{H}}{\partial \mathbf\frakp} + \bfJ_{2}(\mathbf\frakq, \mathbf\frakp)\frac{\partial \mathcal{H}_d}{\partial \mathbf\frakp}\right. \nonumber \\
&& \left.-\bfM_d(\mathbf\frakq)\bfM^{-1}(\mathbf\frakq)\bfR^{\times\top}\frac{\partial \mathcal{H}_d}{\partial \mathbf\frakq}\right). \label{eq:idapbc_u_es} \\
\bfu_{DI}(\mathbf\frakq, \mathbf\frakp) &=& - \bfg^{\dagger} \bfK_d\bfzeta,\label{eq:idapbc_u_di}
\end{eqnarray}
where $\bfg^{\dagger}(\mathbf\frakq) = \left(\bfg^{\top}(\mathbf\frakq)\bfg(\mathbf\frakq)\right)^{-1}\bfg^{\top}(\mathbf\frakq)$ is the pseudo-inverse of $\bfg(\mathbf\frakq)$.





%
%\subsection{Unused}
%For under-actuated systems, we need to shape both potential and kinetic energies in order to drive the system towards the desired state $(\mathbf\frakq^*, \bf0)$. This is done via interconnection and damping assignment passivity-based control approach (IDA-PBC) \cite{van2014port,ortega2002stabilization}. Let $\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp)$ be the desired Hamiltonian:
%\begin{equation}
%\label{eq:desired_hamiltonian}
%\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp) = \frac{1}{2}\mathbf\frakp^\top \bfM_d^{-1}(\mathbf\frakq)\mathbf\frakp + \bfV_d(\mathbf\frakq),
%\end{equation}
%where $\bfM_d(\mathbf\frakq)$ is the desired generalized mass and $\bfV_d(\mathbf\frakq)$ is the desired generalized potential energy such that $\mathbf\frakq^* = \text{argmin}\bfV_d(\mathbf\frakq)$. 
%
%
%
%
%The damping injection control is the same as for fully-actuated system . The energy-shaping control is as follows.
%
%where the desired generalized mass $\bfM_d(\mathbf\frakq)$ and 
%
%
%




\subsection{Controller for fully-actuated systems}
\label{subsec:control_fa}
For fully-actuated systems, we use energy-shaping and damping injection (ES-DI) approach \cite{van2014port} to design our controller. Since the energy $\mathcal{H}(\mathbf\frakq, \mathbf\frakp)$ does not necessarily have a minimum at $(\mathbf\frakq^*, 0)$, the key idea is to add an extra energy $\mathcal{H}_a(\mathbf\frakq, \mathbf\frakp)$ such that the total desired energy $\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp)$ achieves its minimum at $(\mathbf\frakq^*, 0)$:
\begin{equation}
\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp) = \mathcal{H}(\mathbf\frakq, \mathbf\frakp) + \mathcal{H}_a(\mathbf\frakq, \mathbf\frakp).
\end{equation}
The extra energy $\mathcal{H}_a(\mathbf\frakq, \mathbf\frakp)$ satisfies the matching equation \cite{van2014port}:
\begin{equation}
\label{eq:esdi_matching}
\begin{bmatrix}
\mathcal{G}^{\perp}(\mathbf\frakq, \mathbf\frakp)(\bf\mathcal{J}(\mathbf\frakq, \mathbf\frakp) - \bf\mathcal{R}(\mathbf\frakq, \mathbf\frakp)) \\
\mathcal{G}^\top(\mathbf\frakq, \bf\mathfrak{p})
\end{bmatrix}\begin{bmatrix}
\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakq} \\
\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakp} 
\end{bmatrix} = \bf0
\end{equation}
where $\mathcal{G}^{\perp}(\mathbf\frakq, \mathbf\frakp)$ is a maximal-rank left annihilator of $\mathcal{G}(\mathbf\frakq, \mathbf\frakp)$, i.e. $\mathcal{G}^{\perp}(\mathbf\frakq, \mathbf\frakp)\mathcal{G}(\mathbf\frakq, \mathbf\frakp) = \bf0$. When the system is fully actuated, i.e. $\dim(\mathfrak{p}) = \dim(u)$, the matching equation \eqref{eq:esdi_matching} for our learned dynamics (Eq. \eqref{eq:port_Hal_dyn}) is satisfied if $\frac{\partial \mathcal{H}}{\partial\mathbf\frakp} = \bf0$. Therefore, it is enough for the extra energy $\mathcal{H}_a$ to shape the potential energy only.

Given an extra energy $\mathcal{H}_a(\mathbf\frakq, \mathbf\frakp)$ that satisfies the matching equation \eqref{eq:esdi_matching} and makes the total energy $\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp)$ have a minimum at $(\mathbf\frakq^*, 0)$, the state-feedback control is derived as $\bfu(\mathbf\frakq, \mathbf\frakp) = \bfu_{ES}(\mathbf\frakq, \mathbf\frakp)+ \bfu_{DI}(\mathbf\frakq, \mathbf\frakp)$ \cite{van2014port} where
\begin{eqnarray}
\bfu_{ES}(\mathbf\frakq, \mathbf\frakp) &=& \mathcal{G}^{\dagger}(\mathbf\frakq, \mathbf\frakp)(\bf\mathcal{J}(\mathbf\frakq, \mathbf\frakp)-\bf\mathcal{R}(\mathbf\frakq, \mathbf\frakp))\begin{bmatrix}
\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakq} \\
\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakp} 
\end{bmatrix} \label{eq:u_ES_SO3}\\
\bfu_{DI}(\mathbf\frakq, \mathbf\frakp) &=& -\bfK_d\mathcal{G}^\top(\mathbf\frakq, \mathbf\frakp)\begin{bmatrix}
\frac{\partial \mathcal{H}_d}{\partial\mathbf\frakq} \\
\frac{\partial \mathcal{H}_d}{\partial\mathbf\frakp} 
\end{bmatrix}, \label{eq:u_DI_SO3}
\end{eqnarray}
where $\mathcal{G}^{\dagger}(\mathbf\frakq, \mathbf\frakp) = (\mathcal{G}^\top(\mathbf\frakq, \mathbf\frakp)\mathcal{G}(\mathbf\frakq, \mathbf\frakp))^{-1}\mathcal{G}^\top(\mathbf\frakq, \mathbf\frakp)$ is the pseudo-inverse matrix of $\mathcal{G}(\mathbf\frakq, \mathbf\frakp)$. 
%\subsubsection{Attitude control on SO(3) manifold}
%\label{subsubsec:attitude_control_SO3}
%Let $\bfR^{*\top}$ be the desired rotation matrix. Similar to \cite{forni2015port}, we choose the function $\mathcal{H}_a$ as follows.
%\begin{equation}
%\label{eq:H_a_SO3}
%\mathcal{H}_a(\mathbf\frakq, \mathbf\frakp) = -\bfV(\bfR) + \frac{1}{2} \tr(\bfK_{\bfR}(\bfI - \bfR^{*\top}\bfR)).
%\end{equation}
%Then, we have $\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakq} = -\frac{\partial V(\bfR)}{\partial \bfR} - \bfR^*\bfK_{\bfR}^\top$, and $\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakp} = \bf0$. As a result, the total desire Hamiltonian
%\begin{eqnarray}
%\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp) &=& \mathcal{H}(\mathbf\frakq, \mathbf\frakp) + \mathcal{H}_a(\mathbf\frakq, \mathbf\frakp) \nonumber \\
%&=& \frac{1}{2}\mathbf\frakp^\top \bfM(\bfR)^{-1} \mathbf\frakp  + \frac{1}{2} \tr(\bfK_{\bfR}(\bfI - \bfR^{*\top}\bfR)), \nonumber
%\end{eqnarray}
%has a minimum at $(\bfR^*, \bf0)$. The energy-shaping and damping injection controls (Eq. \eqref{eq:u_ES_SO3} and \eqref{eq:u_DI_SO3}) become
%
%\begin{eqnarray}
%\bfu_{ES}(\mathbf\frakq, \mathbf\frakp) &=& \bfg^{\dagger}(\mathbf\frakq, \mathbf\frakp)(-\mathfrak{R}^{\times\top})\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakq} \nonumber \\
%&=&  \bfg^{\dagger}(\mathbf\frakq, \mathbf\frakp) \sum_{i = 1}^3 \bfr_i \times \frac{\partial \mathcal{H}_a}{\partial\bf\bfr_i}\\
%\bfu_{DI}(\mathbf\frakq, \mathbf\frakp) &=& -\bfK_d\bfg^\top(\mathbf\frakq, \mathbf\frakp)\frac{\partial \mathcal{H}_d}{\partial\mathbf\frakp} \nonumber \\
%&=& -\bfK_d\bfg^\top(\mathbf\frakq, \mathbf\frakp)\bfomega.
%\end{eqnarray}

%\subsubsection{Pose control on SE(3) manifold}
Consider a rigid body with pose $\bfT$ controlled by a 6-dimensional wrench $\bfu$ (3-dimensional force and 3-dimensional torque), i.e. the system is fully actuated. Let $\bfT^* = (\bfR^*, \bfp^*)$ be the desired pose of a rigid body, i.e. $\mathbf\frakq^* = [\bfr_1^{*\top}, \bfr_2^{*\top}, \bfr_3^{*\top}, \bfp^{*\top}]$. We choose the function $\mathcal{H}_a$ as follows.
\begin{eqnarray}
\mathcal{H}_a(\mathbf\frakq, \mathbf\frakp) &=& -\bfV_{\bftheta_2}(\mathbf\frakq) + \frac{1}{2} \tr(\bfK_{\bfR}(\bfI - \bfR^{*\top}\bfR)) \nonumber \\
&& + \frac{1}{2}(\bfp - \bfp^*)^\top\bfK_\bfp(\bfp - \bfp^*),\label{eq:H_a_SE3}
\end{eqnarray}
where $\bfK_{\bfR} = \text{diag}(k_{r1}, k_{r2}, k_{r3}), \bfK_\bfp = \text{diag}(k_{p1}, k_{p2}, k_{p3})$. Let $\bfDelta_\bfR = \frac{\partial \left(\frac{1}{2} \tr(\bfK_{\bfR}(\bfI - \bfR^{*\top}\bfR))\right)}{\partial \bfR} = -\frac{1}{2}\bfR^* \bfK_\bfR^\top = \begin{bmatrix}
\bfdelta_1 &
\bfdelta_2 &
\bfdelta_3 
\end{bmatrix}^\top$. We have 
\begin{eqnarray}
\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakq} = -\frac{\partial V_{\bftheta_2}(\mathbf\frakq)}{\partial \bf\mathbf\frakq} + \begin{bmatrix}
\bfdelta_1 \\
\bfdelta_2 \\
\bfdelta_3 \\
\bfK_\bfp(\bfp - \bfp^*)
\end{bmatrix},
\end{eqnarray}
and $\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakp} = \bf0$. As a result, the total desired Hamiltonian,
\begin{eqnarray}
\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp) &=& \mathcal{H}(\mathbf\frakq, \mathbf\frakp) + \mathcal{H}_a(\mathbf\frakq, \mathbf\frakp), \nonumber \\
&=& \frac{1}{2}\mathbf\frakp^\top \bfM_{\bftheta_1}^{-1}(\mathbf\frakq) \mathbf\frakp  + \frac{1}{2} \tr(\bfK_{\bfR}(\bfI - \bfR^{*\top}\bfR)) \nonumber \\
&& + \frac{1}{2}(\bfp - \bfp^*)^\top\bfK_\bfp(\bfp - \bfp^*),
\end{eqnarray}
has a minimum at $(\bfT^*, \bf0)$. The energy-shaping and damping injection controls (Eq. \eqref{eq:u_ES_SO3} and \eqref{eq:u_DI_SO3}) become
\begin{eqnarray}
\bfu_{ES}(\mathbf\frakq, \mathbf\frakp) &=& \bfg_{\bftheta_3}^{\dagger}(\mathbf\frakq)(-\bfR^{\times\top})\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakq} \nonumber \\
&=&  \bfg_{\bftheta_3}^{\dagger}(\mathbf\frakq) \begin{bmatrix}
\sum_{i = 1}^3 \bfr_i \times \frac{\partial \mathcal{H}_a}{\partial\bf\bfr_i} \\
- \bfR^\top \frac{\partial \mathcal{H}_a}{\partial\bf\bfp}
\end{bmatrix}, \label{eq:u_es} \\
\bfu_{DI}(\mathbf\frakq, \mathbf\frakp) &=& -\bfK_d\bfg_{\bftheta_3}^\top(\mathbf\frakq)\frac{\partial \mathcal{H}_d}{\partial\mathbf\frakp} \nonumber \\
&=& -\bfK_d\bfg_{\bftheta_3}^\top(\mathbf\frakq)\bfzeta, \label{eq:u_di}
\end{eqnarray}
where $\frac{\partial \mathcal{H}_a}{\partial\bf\bfr_i} = \bfdelta_i$ and $\frac{\partial \mathcal{H}_a}{\partial\bf\bfp} = \bfK_\bfp(\bfp - \bfp^*)$.






\section{Misc}
\label{sec:misc}
\subsection{A Nominal Quadrotor Dynamics}
\label{subsec:nominal_dynamics}
In this section, we model a quadrotor as a rigid body with its pose kinematics shown in Sec. \ref{subsec:SO3_SE3_kinematics}. Let $m$ and $\bfJ \in \mathbb{R}^{3\times 3}$ be the mass and the inertia matrix of the quadrotor in frame $\{B\}$, respectively.

Then, the dynamics of a quadrotor is shown below \cite{mahony2012multirotor}:
\begin{eqnarray}
\dot{\bfx} &=& \bfrho, \label{eq:pos_dyn}\\
m\dot{\bfrho} &=& -mg\bfe_3 + \bfR\bfe_3f, \label{eq:vel_dyn}\\
\dot{\bfR} &=& \bfR \hat{\bfomega}, \label{eq:rotation_dyn}\\
\bfJ\dot{\bfomega} &=& -\bfomega \times \bfJ\bfomega + \tau, \label{eq:omega_dyn}
\end{eqnarray}
where $f,\tau$ denote the force and torque s generated by the rotors, respectively. The force $f$ and torques $\tau$ can be calculated based on the angular velocity of the rotors $\bar{\omega}_i, i = 1,2,3,4$ as follows:
\begin{equation}
\begin{bmatrix}
f \\ \tau_1 \\ \tau_2 \\ \tau_3
\end{bmatrix} = \begin{bmatrix}
c_T & c_T & c_T & c_T \\
0 & dc_T & 0 & -dc_T \\
-dc_T & 0 & dc_T & 0 \\
-c_Q & c_Q & -c_Q & c_Q
\end{bmatrix} \begin{bmatrix}
\bar{\omega}_1^2 \\
\bar{\omega}_2^2 \\
\bar{\omega}_3^2 \\
\bar{\omega}_4^2
\end{bmatrix},
\end{equation}
\TD{Assuming there is no secondary force like drag force here.}, $\bfe_3 = [0,0,1]^\top$, $d$ is the arm length, $c_T$ and $c_Q$ are the thrust and torque coefficients, respectively.
%\subsection{Neural ODE Networks}
%chen2018neural

\subsection{Hamiltonian Dynamics for rotation matrix on SO(3)}
\label{subsec:hamiltonian_dynamics_rotmat}
For dynamics learning purposes, the nominal dynamics of a quadrotor shown in Section \ref{subsec:nominal_dynamics} poses a challenge that the time evolution of the rotation matrix $\bfR$ (Eq. \eqref{eq:rotation_dyn}) is performed on an SO(3) manifold. The manifold constraints might be hard to enforce in learning frameworks such as Neural ODE.

\NEW{\textbf{Remarks:}  Assume that we use a rotation representation $\beta \in \mathbb{R}^{d}$ (e.g. rotation matrix($d=9$), quaternion ($d=4$), Euler angles ($d=3$), a continuous $6$D representation ($d=6$)) and its derivative $\dot{\beta} \in \mathbb{R}^{d}$ in the Hamiltonian dynamics. As shown in Sec. \ref{sec:misc}, for $d > 3$ the matrix $\bfM(\bf\mathfrak{q})$ is an $d\times d$ matrix that has rank $3$ since $\dot{\beta}$ depends on the angular velocity $\bfomega \in \mathbb{R}^3$. Meanwhile, in the Symplectic Neural ODE framework,  the matrix $\bfM(\bf\mathfrak{q})$ is p.s.d and therefore, of full rank. For $d=3$, the matrix $\bfM(\bf\mathfrak{q})$ does have full rank. However, any $3$-dimensional representation of rotation suffers from singularities causing low-rank matrix $\bfM(\bf\mathfrak{q})$ as well.} Therefore, we want to use a representation with $d > 3$ together with angular velocity in Hamiltonian dynamics. In this paper, we use rotation matrix ($d=9$) for representing orientation and leave the other representations with $d>3$ for future work.  However, the Hamiltonian dynamics in this case is on SO(3) manifold instead of $\mathbb{R}^d$ as described in Sec. \ref{subsec:symplectic_neuralode}. In this section, we describe the Hamiltonian dynamics for rotation matrix $\bf\mathfrak{q} = [\bfr_1^\top, \bfr_2^\top, \bfr_3^\top]^\top$ on SO(3) manifold \cite{lee2017global}.

The Lagrangian function for the rotation matrix is the difference between a quadratic kinetic energy in terms of the angular velocity $\bfomega$ and the potential energy $\bfV(\bf\bfR)$.
\begin{equation}
\label{eq:lagrangian_angvel}
L(\bfR, \bfomega) = \frac{1}{2}\bfomega^\top \bfJ \bfomega - \bfV(\bfR),
\end{equation}
 where $\bfJ$ is the inertia matrix. Assume that the matrix $\bfJ$ is unknown and to be learned as a function $\bfJ = \bfM(\bfR)$.  This is called a modified Lagrangian function \cite{lee2017global} since it is written in terms of $\bfR$ and $\bfomega$ instead of $\bf\bfR$ and $\dot{\bfR}$. In other words, the angular velocity $\bfomega \in \mathbb{R}^3$ can be consider as a modified $\dot{\bf\mathfrak{q}}$ and related to $\dot{\bf\mathfrak{q}} = \dot{\bfR}$ in the tangent space of SO(3) according to Eq. \eqref{eq:rotmat_kinematics}.  Using Legendre transformation $\bf\mathfrak{p} = \frac{\partial L(\bfR, \bfomega)}{\partial \bfomega} = \bfM(\bfR) \bfomega$, the Hamiltonian is calculated as follows.
\begin{equation}
\label{eq:hamiltonian_rotmat}
\mathcal{H}(\bfR,\bf\mathfrak{p}) = \bf\mathfrak{p}^\top \bfomega - L(\bfR, \bfomega) = \frac{1}{2}\bf\mathfrak{p}^\top \bfM(\bfR)^{-1} \bf\mathfrak{p} + \bfV(\bfR)
\end{equation}
The Hamilton's equations for the Hamiltonian in Eq. \eqref{eq:hamiltonian_rotmat} are shown below. We refer the readers to \cite{lee2017global} for a detailed derivation.
\begin{eqnarray}
\dot{\bfr_i} &=& \bfr_i \times \frac{\partial{H(\bfR,\bf\mathfrak{p})}}{\partial \bf\mathfrak{p}}, \quad i = 1,2,3 \label{eq:hamiltonian_rotmat_rdot} \\
\dot{\bf\mathfrak{p}} &=& \bf\mathfrak{p} \times \frac{\partial{\mathcal{H}(\bfR,\bf\mathfrak{p})}}{\partial \bf\mathfrak{p}} + \sum_{i = 1}^3 \bfr_i \times \frac{\partial{\mathcal{H}(\bfR,\bf\mathfrak{p})}}{\partial \bfr_i} + \bfg(\bfR)\bfu. \nonumber \\
&&\label{eq:hamiltonian_rotmat_pdot}
\end{eqnarray}
Note that these equations are different from Eq. \eqref{eq:hamiltonian_evolution_control} due to the constraints and kinematics on SO(3) manifold.



\iffalse
For dynamics learning purposes, the nominal dynamics of a quadrotor shown in Section \ref{subsec:nominal_dynamics} poses a challenge that the time evolution of the rotation matrix $\bfR$ (Eq. \eqref{eq:rotation_dyn}) is performed on an SO(3) manifold. The manifold constraints might be hard to enforce in learning frameworks such as Neural ODE. I've been thinking about the following approaches to learn the dynamics on the SO(3) manifold.

\begin{itemize}
\item \textbf{Using unit quaternion}: this replaces SO(3) constraints with simpler ones for quaternion. We  re-formulate the Hamiltonian function for the quaternion (Section \ref{subsec:hamiltonian_unit_quaternion}) and enforce unit quaternion at every step or at the end of ODE solvers.
\item \textbf{Using non-unit quaternion}: this does not have any constraints. We  re-formulate the Hamiltonian function for the quaternion (Section \ref{subsec:hamiltonian_nonunit_quaternion}). However, we need to normalize the quaternion and/or convert back to rotation matrix when calculating loss function.
\item \textbf{Using continuous $6$D representation}: the problem of quaternions is that they are discontinuous leading to high error occasionally. We  re-formulate the Hamiltonian function for the continuous $6$D representation (Section \ref{subsec:hamiltonian_continuous_6d}). This might help with learning process but we need to perform Gram-Schmit-like normalization and convert to rotation matrix for loss function.
\item \textbf{Using Euler angles}: this will get rid of SO(3) constraints. We re-formulate the Hamiltonian function for the Euler angles (\textbf{done} in Section \ref{subsec:hamiltonian_euler_angles}). However, it suffers from singularity issues.
\end{itemize}
\subsection{Hamiltonian dynamics formulation for quadrotor dynamics with unit quaternions}
\label{subsec:hamiltonian_unit_quaternion}
In this section, we re-write the Hamiltonian dynamics in terms of unit quaternions and effectively replace the SO(3) constraints with simpler constraint of a unit quaternion. Let $\bfbeta = [\beta_0, \beta_1, \beta_2, \beta_4]$ be the quaternion representing the rotation matrix $\bfR$. A quaternion $\bfbeta$ has to satisfy the following constraint:
\begin{equation}
\label{eq:quat_constraint}
\bfbeta^\top \bfbeta = 1
\end{equation}
Eq. \eqref{eq:rotation_dyn} can be rewritten for quaternion as follows \cite{faessler2015automatic, falanga2018pampc}:
\begin{equation}
\label{eq:quat_dyn}
\dot{\bfbeta} = \frac{1}{2}\bfLambda(\bfomega)\bfbeta,
\end{equation}
where $\bfLambda = \begin{bmatrix}
0        & -\omega_1 & -\omega_2 & -\omega_3 \\
\omega_1 &         0 &  \omega_3 & -\omega_2 \\
\omega_2 & -\omega_3& 0& \omega_1 \\
\omega_3 & \omega_2& -\omega_1& 0 
\end{bmatrix}.$

Eq. \eqref{eq:quat_dyn} has the angular velocity in the form of a matrix $\bfLambda$ making it hard to integrate into Hamiltonian function. Shivarama and Fahrenlhold \cite{shivarama2004hamilton} look at quaternion from an Euler parameters perspective, rewrite Eq. \eqref{eq:quat_dyn} as
\begin{equation}
\label{eq:quat_dyn_hamiltonian}
\dot{\bfbeta} = \frac{1}{2}\bfK(\bfbeta) \bfomega.
\end{equation}
where $\bfK(\bfbeta) = \begin{bmatrix}
-\beta_1 & -\beta_2 & -\beta_3 \\
 \beta_0 & -\beta_3 &  \beta_2 \\
 \beta_3 &  \beta_0 & -\beta_1 \\
-\beta_2 &  \beta_1 &  \beta_0
\end{bmatrix}, $
and derive a Hamiltonian dynamics for rigid body with quaternion. Note that $\bfK(\bfbeta)^\top \bfK(\bfbeta) = \bfI$ so 
\begin{equation}
\label{eq:unit_quad_omega_dyn_hamiltonian}
\bfomega = 2\bfK(\bfbeta)^\top \dot{\bfbeta},
\end{equation}
where $\bfbeta$ is a unit quaternion.
Similar to Section \ref{subsec:hamiltonian_dynamics_rotmat} and \cite{shivarama2004hamilton}, we define the state $\bfq = [\bfxi^\top, \bfbeta^\top]^\top$, $\dot{\bfq} = [\dot{\bfxi}^\top, \dot{\bfbeta}^\top]^\top$, and 
\begin{equation}
\bfM(\bfq) = \begin{bmatrix}
m\bfI & 0 \\
0 & 4\bfK(\bfbeta)\bfJ \bfK(\bfbeta)^\top 
\end{bmatrix} \in \mathbb{R}^{7\times7}
\end{equation}
Now, Eq. \eqref{eq:hamiltonian_quad} also holds with $\bfp = \frac{\partial L(\bfq, \dot{\bfq})}{\partial \dot{\bfq}} = \bfM(\bfq) \dot{\bfq}$.

\TODO{Remarks: The problem of this approach is that the $\bfK(\bfbeta)\bfJ \bfK(\bfbeta)^\top \in \mathbb{R}^{4\times 4}$ but only has rank 3. Meanwhile, we try to approximate this matrix by a $4\times 4$ p.s.d matrix leading to high errors.}
\subsection{Hamiltonian dynamics formulation for quadrotor dynamics with non-unit quaternions}
\label{subsec:hamiltonian_nonunit_quaternion}
Rucker \cite{rucker2018integrating} showed that if a non-unit quaternion $\bfbeta$ is used instead to represent the rotation matrix, the constraints for unit quaternion does not need to be enforced in ODE solvers such as Runge-Kutta method. Eq. \eqref{eq:unit_quad_omega_dyn_hamiltonian} now becomes:
\begin{equation}
\label{eq:nonunit_quad_omega_dyn_hamiltonian}
\bfomega = \frac{2}{\Vert\bfbeta\Vert^2}\bfK(\bfbeta)^\top \dot{\bfbeta},
\end{equation}
However, when the non-unit quaternion $\bfbeta$ approaches $0$ (since it's not being normalized at every step), ODE solvers might be numerically unstable. To improve on this, Rucker \cite{rucker2018integrating} derived a general solution to Eq. \eqref{eq:nonunit_quad_omega_dyn_hamiltonian}:
\begin{equation}
\label{eq:nonunit_quat_dyn_hamiltonian}
\dot{\bfbeta} = \frac{\Vert\bfbeta\Vert^2}{2}\bfK(\bfbeta) \bfomega + c\bfbeta \quad \forall c \in \mathbb{R}.
\end{equation}
since $\bfbeta \in \textbf{null}(\bfK(\bfbeta)^\top)$. The scalar $c$ is varied to make the gradient more stable when $\bfbeta$ is close to $0$. In \cite{rucker2018integrating}, it is set to $c = k(1-\Vert\bfbeta\Vert)$ even though it should hold for all $c\in \mathbb{R}$. For $c \neq 0$, Rucker \cite{rucker2018integrating} expected the non-unit quaternion dynamics (Eq. \eqref{eq:nonunit_quat_dyn_hamiltonian}) to violate the law of conservation of energy but the experiments did not seem to agree. However, I think it is actually makes sense to expect conservation of energy in this case. Indeed, let $\bfbeta' = \frac{\bfbeta}{\Vert \bfbeta \Vert}$. We have $\dot{\bfbeta'} = \left(\bfI - \bfbeta' \bfbeta'^\top\right)\frac{\dot{\bfbeta}}{\Vert \bfbeta\Vert}$, and therefore, $\bfK(\bfbeta')^\top \dot{\bfbeta'} = \bfK(\bfbeta')^\top\frac{\dot{\bfbeta}}{\Vert\bfbeta\Vert}$ since $\bfbeta' \in \textbf{null}(\bfK(\bfbeta')^\top)$. From Eq. \eqref{eq:nonunit_quat_dyn_hamiltonian}, we can find the angular velocity as follows.
\begin{eqnarray}
\bfomega &=& \frac{2}{\Vert\bfbeta\Vert^2}\bfK(\bfbeta)^\top \dot{\bfbeta}\\
&=& 2\bfK(\bfbeta')^\top \frac{\dot{\bfbeta}}{\Vert\bfbeta\Vert} \nonumber \\
&=& 2\bfK(\bfbeta')^\top\dot{\bfbeta'} 
\end{eqnarray}
since $\bfbeta \in \textbf{null}(\bfK(\bfbeta)^\top)$. This is exactly Eq. \eqref{eq:unit_quad_omega_dyn_hamiltonian} with the unit quaternion $\bfbeta'$. In other words, regardless of $c$ and multiple non-unit quaternions $\bfbeta$ representing the same rotation, the angular velocity only depends on the normalized quaternion $\bfbeta'$, and hence, the Lagrangian function is still a constant given zero control input.

Similar to Section \ref{subsec:hamiltonian_dynamics_rotmat} and \cite{shivarama2004hamilton}, we define the state $\bfq = [\bfxi^\top, \bfbeta^\top]^\top$, $\dot{\bfq} = [\dot{\bfxi}^\top, \dot{\bfbeta}^\top]^\top$, and 
\begin{equation}
\bfM(\bfq) = \begin{bmatrix}
m\bfI & 0 \\
0 & \frac{4}{\Vert\bfbeta\Vert^4}\bfK(\bfbeta)\bfJ \bfK(\bfbeta)^\top 
\end{bmatrix} \in \mathbb{R}^{7\times7}
\end{equation}
Now, Eq. \eqref{eq:hamiltonian_quad} also holds with $\bfp = \frac{\partial L(\bfq, \dot{\bfq})}{\partial \dot{\bfq}} = \bfM(\bfq) \dot{\bfq}$.

\textbf{Remarks.} This means we don't need to normalized $\bfbeta$ inside ODE solver. \TODO{However, the problem of this approach is that the $\bfK(\bfbeta)\bfJ \bfK(\bfbeta)^\top \in \mathbb{R}^{4\times 4}$ but only has rank 3. Meanwhile, we try to approximate this matrix by a $4\times 4$ p.s.d matrix leading to high errors.}


\subsection{Hamiltonian dynamics formulation for quadrotor dynamics with continuous 6D representation for rotation matrix}
\label{subsec:hamiltonian_continuous_6d}

Zhou et. al. \cite{zhou2019continuity} used results from topology to show that any rotation matrix representation with less than or equal to $4$ dimensions is discontinuous making it hard for learning the rotation dynamics. They proposed a $6$D representation by extracting the first two columns $\bfb_x, \bfb_y$ of the rotation matrix $\bfR$ and set the third column $\bfb_z = \bfb_x \times \bfb_y$. The constraints for this $6$D representation are: $\Vert\bfb_x\Vert = 1, \Vert\bfb_y\Vert = 1$ and $\bfb_x^\top\bfb_y = 0$. We now need to derive the Hamiltonian function in terms of this $6$D representation $\bfgamma = [\bfb_x^\top, \bfb_y^\top]^\top$ by relating the angular velocity $\bfomega$ to $\dot{\bfgamma}$.

Given $\bfgamma = [\bfb_x^\top, \bfb_y^\top]^\top$, we have:
\begin{equation}
\bfb_z = \bfb_x \times \bfb_y = \begin{bmatrix}
b_{x2}b_{y3} - b_{x3}b_{y2} \\
b_{x3}b_{y1} - b_{x1}b_{y3} \\
b_{x1}b_{y2} - b_{x2}b_{y1} 
\end{bmatrix},
\end{equation}
and
\begin{equation}
\dot{\bfR}_f = \bfP(\bfgamma)\dot{\bfgamma}
\end{equation}
where $\bfR_f \in \mathbb{R}^9$ is the flattened (column-wise) version of the rotation matrix and $\bfP(\bfgamma) = \begin{bmatrix}
&&\bfI_{6\times6} \\
0 & b_{y3} & -b_{y2} & 0 & -b_{x3} & b_{x2} \\
-b_{y3} & 0 & b_{y1} & b_{x3} & 0 & -b_{x1} \\
b_{y2} & -b_{y1} & 0 & -b_{x2} & b_{x1} & 0 \\
\end{bmatrix}\in \mathbb{R}^{9\times 6}$.
Similarly, Eq. \eqref{eq:rotation_dyn} can be re-written with flattened $\bfR_f \in \mathbb{R}^9$ as follows.
\begin{equation}
\dot{\bfR}_f = \bfQ(\bfgamma)\bfomega
\end{equation}
where $\bfQ(\bfgamma) = \begin{bmatrix}
\bf0 & -\bfb_x\times \bfb_y & \bfb_y \\
\bfb_x\times \bfb_y & 0 & -\bfb_x \\
-\bfb_y & \bfb_x & \bf0
\end{bmatrix} \in \mathbb{R}^{9\times 3}.$ Note that $\bfQ(\bfgamma)^\top \bfQ(\bfgamma) = 2\bfI_{3\times 3}$. Therefore, one can easily relate the angular velocity with $\dot{\bfgamma}$.
\begin{equation}
\label{eq:6d_omega_dyn_hamiltonian}
\bfomega = \frac{1}{2}\bfQ(\bfgamma)^\top \bfP(\bfgamma)\dot{\bfgamma},
\end{equation}
and 
\begin{equation}
\label{eq:6d_gammadot_dyn_hamiltonian}
\dot{\bfgamma} = \bfQ'(\bfgamma)\bfomega,
\end{equation}
where $\bfQ'(\bfgamma) = \begin{bmatrix}
\bf0 & -\bfb_x\times \bfb_y & \bfb_y \\
\bfb_x\times \bfb_y & 0 & -\bfb_x
\end{bmatrix} \in \mathbb{R}^{6\times 3}$ which is the top $6$ rows of $\bfQ$.

Similar to Section \ref{subsec:hamiltonian_dynamics_rotmat} and \cite{shivarama2004hamilton}, we define the state $\bfq = [\bfxi^\top, \bfgamma^\top]^\top$, $\dot{\bfq} = [\dot{\bfxi}^\top, \dot{\bfgamma}^\top]^\top$, and 
\begin{equation}
\bfM(\bfq) = \begin{bmatrix}
m\bfI & 0 \\
0 & \frac{1}{4}\bfP(\bfgamma)^\top \bfQ(\bfgamma) \bfJ \bfQ(\bfgamma)^\top \bfP(\bfgamma) 
\end{bmatrix} \in \mathbb{R}^{10\times10}
\end{equation}
Now, Eq. \eqref{eq:hamiltonian_quad} also holds with $\bfp = \frac{\partial L(\bfq, \dot{\bfq})}{\partial \dot{\bfq}} = \bfM(\bfq) \dot{\bfq}$.

\TODO{Remarks: The problem of this approach is that the $\bfP(\bfgamma)^\top \bfQ(\bfgamma) \bfJ \bfQ(\bfgamma)^\top \in \mathbb{R}^{6\times 6}$ but only has rank 3. Meanwhile, we try to approximate this matrix by a $4\times 4$ p.s.d matrix leading to high errors.}


\subsection{Using Euler angles instead of rotation matrix in quadrotor dynamics}
\label{subsec:hamiltonian_euler_angles}
Similar to \cite{wu2018modeling}, we eliminate the SO(3) constraints on the rotation matrix $R$ (Eq. \eqref{eq:rotation_dyn}) by using Euler angles $\bfeta = [\phi, \theta, \psi]^\top$ of roll ($\phi$), pitch ($\theta$), and yaw angles ($\psi$) (i.e. ``XYZ" extrinsic rotation). This representation allows us to relate the roll, pitch, and yaw rates with the angular velocity $\bfOmega$ as follows (\cite{o2008intermediate}, page 188 \TD{According to \href{http://personal.maths.surrey.ac.uk/T.Bridges/SLOSH/3-2-1-Eulerangles.pdf}{this pdf}}, (\TODO{Q:Does this hold with Gimbal locks?})).
\begin{equation}
\label{eq:omega_rpy_rates}
\bfOmega = \begin{bmatrix}
1 & 0 & -\sin{\theta} \\
0 & \cos{\phi} & \cos{\theta}\sin{\phi} \\
0 & -\sin{\phi} & \cos{\theta}\cos{\phi}
\end{bmatrix} \begin{bmatrix}
\dot{\phi} \\
\dot{\theta} \\
\dot{\psi}
\end{bmatrix} = \bfK(\bfeta)\dot{\bfeta}
\end{equation}
Plugging Eq. \eqref{eq:omega_rpy_rates} into Eq. \eqref{eq:lagrangian_angvel}, we have:
\begin{equation}
\label{eq:lagrangian_rpy}
L(\bfq, \dot{\bfq}) = \frac{1}{2}m\dot{\bfxi}^\top \bfI \dot{\bfxi} + \frac{1}{2}\dot{\bfeta}^\top \bfK(\bfeta)^\top \bfJ \bfK(\bfeta)\dot{\bfeta} + mgz
\end{equation}

Now, let define $\bfq = [\bfxi^\top, \bfeta^\top]^\top, \dot{\bfq} = [\dot{\bfxi}^\top, \dot{\bfeta}^\top]^\top$, and

\begin{equation}
\bfM(\bfq) = \begin{bmatrix}
m\bfI & 0 \\
0 & \bfK(\bfeta)^\top \bfJ \bfK(\bfeta)
\end{bmatrix} \in \mathbb{R}^{6\times6}
\end{equation}

(\TODO{$\bfK(\bfeta)$ is not of full rank if $\theta = \pm \frac{\pi}{2}$ (singularities) so $\bfM(\bfq)$ might not be invertible. Does this matter as we use a neural network to directly learn this matrix inverse anyway?})

Notice that Eq. \eqref{eq:hamiltonian_quad} has the same form as Eq. \eqref{eq:hamiltonian_def}. \textbf{Consequently, this allows us to use the symplectic neural ode learning framework described in Section \ref{subsec:symplectic_neuralode} to learn the dynamics of quadrotors with states $\bfq = [\bfxi^\top, \bfeta^\top]^\top$, i.e. using Euler angles instead of rotation matrix.} This effective replaces complicated SO(3) manifold constraints with simpler Euler angle constraints $\phi, \theta, \psi \in [-\pi, \pi]$. Zhong et. al. \cite{zhong2020symplectic} already proposed a trick to work around this kind of constraints which replace an angle, e.g. $\phi$, by its sin and cosin, e.g. $\sin{\phi}, \cos{\phi}$ in the dynamics.
\begin{equation}
\dot{\sin{\phi}} = \cos{\phi}\dot{\phi}, \qquad
\dot{\cos{\phi}} = -\sin{\phi}\dot{\phi}
\end{equation}

\textbf{Remarks}: We might have singularity with Euler angles. As a result, $\bfK(\bfeta)^\top \bfJ \bfK(\bfeta)$ have rank lower than $3$.

\fi

==> tex/unused2.tex <==
\section{Misc}
\label{sec:misc}
\subsection{A Nominal Quadrotor Dynamics}
\label{subsec:nominal_dynamics}
In this section, we model a quadrotor as a rigid body with its pose kinematics shown in Sec. \ref{subsec:SO3_SE3_kinematics}. Let $m$ and $\bfJ \in \mathbb{R}^{3\times 3}$ be the mass and the inertia matrix of the quadrotor in frame $\{B\}$, respectively.

Then, the dynamics of a quadrotor is shown below \cite{mahony2012multirotor}:
\begin{eqnarray}
\dot{\bfx} &=& \bfrho, \label{eq:pos_dyn}\\
m\dot{\bfrho} &=& -mg\bfe_3 + \bfR\bfe_3f, \label{eq:vel_dyn}\\
\dot{\bfR} &=& \bfR \hat{\bfomega}, \label{eq:rotation_dyn}\\
\bfJ\dot{\bfomega} &=& -\bfomega \times \bfJ\bfomega + \tau, \label{eq:omega_dyn}
\end{eqnarray}
where $f,\tau$ denote the force and torque s generated by the rotors, respectively. The force $f$ and torques $\tau$ can be calculated based on the angular velocity of the rotors $\bar{\omega}_i, i = 1,2,3,4$ as follows:
\begin{equation}
\begin{bmatrix}
f \\ \tau_1 \\ \tau_2 \\ \tau_3
\end{bmatrix} = \begin{bmatrix}
c_T & c_T & c_T & c_T \\
0 & dc_T & 0 & -dc_T \\
-dc_T & 0 & dc_T & 0 \\
-c_Q & c_Q & -c_Q & c_Q
\end{bmatrix} \begin{bmatrix}
\bar{\omega}_1^2 \\
\bar{\omega}_2^2 \\
\bar{\omega}_3^2 \\^{-1}
\bar{\omega}_4^2
\end{bmatrix},
\end{equation}
\TD{Assuming there is no secondary force like drag force here.}, $\bfe_3 = [0,0,1]^\top$, $d$ is the arm length, $c_T$ and $c_Q$ are the thrust and torque coefficients, respectively.
%\subsection{Neural ODE Networks}
%chen2018neural

\subsection{Hamiltonian Dynamics for rotation matrix and attitude control}
\label{subsec:hamiltonian_dynamics_rotmat}
For SO(3), the Eq. \eqref{eq:hamiltonian_pose_rdot}, \eqref{eq:hamiltonian_pose_pdot}, \eqref{eq:hamiltonian_pose_pomegadot}, \eqref{eq:hamiltonian_pose_pvdot} reduce to:
\begin{eqnarray}
\dot{\bfr_i} &=& \bfr_i \times \frac{\partial{H(\mathbf\frakq,\bf\mathfrak{p})}}{\partial \bf\mathfrak{p}_{\bfomega}}, \quad i = 1,2,3 \label{eq:hamiltonian_rotmat_rdot} \\
\dot{\bf\mathfrak{p}}_{\bfomega} &=& \bf\mathfrak{p}_{\bfomega} \times \frac{\partial{\mathcal{H}(\mathbf\frakq,\bf\mathfrak{p})}}{\partial \bf\mathfrak{p}_{\bfomega}} + \sum_{i = 1}^3 \bfr_i \times \frac{\partial{\mathcal{H}(\mathbf\frakq,\bf\mathfrak{p})}}{\partial \bfr_i} + \bfg_{\bfomega}(\mathbf\frakq)\bfu. \nonumber \\
&& - \bfD_{\bfomega}(\mathbf\frakq, \mathbf\frakp)\frac{\partial{\mathcal{H}(\mathbf\frakq, \mathbf\frakp)}}{\partial \mathbf\frakp_{\bfomega}} \label{eq:hamiltonian_rotmat_pdot}
\end{eqnarray}

For controllers, the additional energy with $\mathbf\frakp = \mathbf\frakp_{\bfomega}$ is:
\begin{equation}
\mathcal{H}_a(\mathbf\frakq, \mathbf\frakp) = -\bfV_{\bftheta_2}(\mathbf\frakq) + \frac{1}{2} \tr(\bfK_{\bfR}(\bfI - \bfR^{*\top}\bfR)).
\end{equation}
The desired Hamiltonian function becomes
\begin{eqnarray}
\mathcal{H}_d(\mathbf\frakq, \mathbf\frakp) &=& \mathcal{H}(\mathbf\frakq, \mathbf\frakp) + \mathcal{H}_a(\mathbf\frakq, \mathbf\frakp), \nonumber \\
&=& \frac{1}{2}\mathbf\frakp^\top \bfM_{\bftheta_1}^{-1}(\mathbf\frakp) \mathbf\frakp  + \frac{1}{2} \tr(\bfK_{\bfR}(\bfI - \bfR^{*\top}\bfR)), \nonumber
\end{eqnarray}
has a minimum at $(\bfT^*, \bf0)$. The energy-shaping and damping injection controls (Eq. \eqref{eq:u_ES_SO3} and \eqref{eq:u_DI_SO3}) become
\begin{eqnarray}
\bfu_{ES}(\mathbf\frakq, \mathbf\frakp) &=& \bfg_{\bftheta_3}^{\dagger}(\mathbf\frakq)(-\bfR^{\times\top})\frac{\partial \mathcal{H}_a}{\partial\mathbf\frakq} \nonumber \\
&=&  \bfg_{\bftheta_3}^{\dagger}(\mathbf\frakq) \sum_{i = 1}^3\bfr_i \times \frac{\partial \mathcal{H}_a}{\partial\bf\bfr_i} \label{eq:u_es} \\
\bfu_{DI}(\mathbf\frakq, \mathbf\frakp) &=& -\bfK_d\bfg_{\bftheta_3}^\top(\mathbf\frakq)\frac{\partial \mathcal{H}_d}{\partial\mathbf\frakp} \nonumber \\
&=& -\bfK_d\bfg_{\bftheta_3}^\top(\mathbf\frakq)\bfomega. \label{eq:u_di}
\end{eqnarray}


